Analysis and computations of a stochastic Cahn-Hilliard model for tumor growth with chemotaxis and variable mobility

In this work, we present and analyze a system of PDEs, which models tumor growth by considering chemotaxis, active transport, and random effects. The stochasticity of the system is modelled by random initial data and Wiener noises that appear in the tumor and nutrient equations. The volume fraction of the tumor is governed by a stochastic phase-field equation of Cahn-Hilliard type, and the mass density of the nutrients is modelled by a stochastic reaction-diffusion equation. We allow a variable mobility function and non-increasing growth functions, such as logistic and Gompertzian growth. Via approximation and stochastic compactness arguments, we prove the existence of a probabilistic weak solution and, in the case of constant mobilities, the well-posedness of the model in the strong probabilistic sense. Lastly, we propose a numerical approximation based on the Galerkin finite element method in space and the semi-implicit Euler-Maruyama scheme in time. We illustrate the effects of the stochastic forcing in the tumor growth in several numerical simulations.

==> 1_model.tex <==
\section{Mathematical model}
\label{Sec:Model}
 








==> C_app.tex <==
\section{Limit passage}

From the uniform estimates \eqref{est1}--\eqref{est4} obtained above, 
there exists a constant $M$, independent of $\lambda$, such that
\begin{equation}\label{uniform_bounds_lambda}
\begin{split}
\norm{\sigmal}_{L^p(\Omega;\! C^0([0,T];\! H)\cap L^2(0,T;\! V))\cap L^\infty(\Omega\times Q)} &\leq M, \\
\norm{\phil}_{L^p(\Omega;\! C^0([0,T];\! H)\cap L^\infty(0,T;\! V)\cap L^2(0,T;\! H^2_N(D)))} &\leq M , \\
\norm{\mul}_{L^{p/2}(\Omega;\! L^2(0,T;\! V))}+
\norm{\nabla \mul}_{L^p(\Omega;\! L^2(0,T;\! H))}
+\norm{(\mul)_D}_{L^{p/2}(\Omega;\! L^\infty(0,T))} &\leq M ,\\
\norm{\Psi'_\lambda(\phil)}_{L^{p/2}(\Omega;\! L^2(0,T;\! H))} &\le M.
\end{split}
\end{equation} 
Moreover, given $s \in (0,1/2)$, from Hypothesis (A3) and \cite[Lem.~2.1]{flandoli1995martingale} 
$$
G \cdot W_1 \in L^p(\Omega;\! W^{s,2}(0,T;\!V)) \cap L^\kappa(\Omega;\! W^{s,\kappa}(0,T);\!V')) 
\quad \forall  \kappa \geq 2,
$$
and by comparison in \eqref{eq_phi_weak} it holds that 
\begin{equation*}
\| \phil \|_{L^p(\Omega;\! W^{s,\kappa}(0,T;\!V'))} \leq M.
\end{equation*}
This is crucial when dealing with the method of compactness:
fixing $\kappa >\frac{1}{s}$, by \cite[Cor.~4-5]{simon1986compact} the following inclusions are compact
\begin{equation*}
\begin{split}
L^\infty(0,T;\!V) \cap W^{s,\kappa}(0,T;\!V') &\hookrightarrow C^0([0,T];\!H), \\
L^2(0,T;\! H^2_N(D)) \cap W^{s,2}(0,T;\!V') &\hookrightarrow L^2(0,T;\!V).
\end{split}
\end{equation*}
We are now in position to show that the family of laws 
$(\pi_\lambda)_{\lambda} := (\calL(\phil))_\lambda$ is a tight family of
probability measures on $C([0,T];\! H) \cap L^2(0,T;\! V)$. 
Denoting $\mathcal{X}:= L^\infty(0,T;\!V) \cap W^{s,\kappa}(0,T;\!V') \cap L^2(0,T;\! H^2_N(D))$, 
we know that $\mathcal{X} \hookrightarrow C([0,T];\! H) \cap L^2(0,T;\! V)$ compactly and
$$ \| \phil \|_{L^p(\Omega;\! \mathcal{X})} \leq M.$$ 
Hence, denoting by $B_n$ the closed ball of radius $n$ in $\mathcal X$,
we have that $B_n$ is compact in $C([0,T];\! H) \cap L^2(0,T;\! V)$ and
the Markov inequality implies that
$$
  \sup_{\lambda>0}\pi_\lambda(B_n^c)=
  \sup_{\lambda>0}\bbP\{\norm{\phil}_{\mathcal X}^p>n^p\}
  \leq \frac1{n^p}\bbE\norm{\phil}_{\mathcal X}^p\leq \frac{M^p}{n^p}\to 0
$$
as $n\to\infty$. We deduce that for every $\varepsilon >0$
there is $n\in\bbN$ sufficiently large such that the compact 
set $B_n$ of $C([0,T];\! H) \cap L^2(0,T;\! V)$ satisfies
$\pi_\lambda(B_n) > 1-\varepsilon$ for every $\lambda>0$, and this proves the tightness of the laws 
$(\pi_\lambda)_\lambda$ on $C([0,T];\! H) \cap L^2(0,T;\! V)$.

In order to reconstruct a process from the limit law, we need to exhibit a 
random variable $\phi: (\Omega,\calF,\bbP) \to C([0,T];\! H) \cap L^2(0,T;\! V)$ 
such that for every $\delta > 0$
$$\bbP\{\|\phil - \phi\|_{C([0,T];\! H) \cap L^2(0,T;\! V)} > \delta\}
\longrightarrow 0 \quad \text{ as } \lambda \to 0. $$
Thanks to the Gy\"ongy-Krylov lemma, see \cref{Lem:GyongyKrylov},
this is equivalent to the following:
for any subsequences $(\phi_{k})_k:= (\phi_{\lambda_k})_k$ and 
$(\phi_{j})_j := (\phi_{\lambda_j})_j$ of the original sequence 
$(\phi_{\lambda})_\lambda$, there exists a joint subsequence 
$(\phi_{k_i}, \phi_{j_i})_i$ converging in law to a probability 
measure $\nu$ on $(C([0,T];\! H) \cap L^2(0,T;\! V))^2$ with the property
\begin{equation}\label{crit_G-K}
\nu \left(  \left\lbrace (g^1,g^2) \in (C([0,T];\! H) \cap L^2(0,T;\! V))^2 : 
g^1 = g^2 \right\rbrace \right) = 1. 
\end{equation} 
Let us now prove the validity of \eqref{crit_G-K}.
Using the tightness of the laws $(\pi_\lambda)_\lambda$ and 
Skorokhod theorem, see \cref{Lem:Skorohod}, we can find a new probability space 
$(\tilde \Omega, \tilde \calF, \tilde \bbP)$ along with a sequence of 
random variables $(\tilde \phi_{k_i},\tilde \phi_{j_i}) : 
\tilde \Omega \to (C([0,T];\! H) \cap L^2(0,T;\! V))^2$ such that 
\begin{equation}\label{conv_skorohod}
(\tilde \phi_{k_i},\tilde \phi_{j_i}) \longrightarrow 
(\phi^1, \phi^2) \qquad \text{ in } (C([0,T];\! H) \cap L^2(0,T;\! V))^2, \quad \tilde \bbP\text{-a.s. }
\end{equation}
and $\mathscr{L}(\phi_{k_i}, \phi_{j_i}) = 
\mathscr{L}(\tilde \phi_{k_i}, \tilde \phi_{j_i})$, for every $i \in \bbR$.
Moreover, there exists a sequence of measurable maps 
$\Upsilon_i: (\tilde \Omega, \tilde \calF) \to (\Omega, \calF)$ 
such that for every $i \in \bbR$ it holds that $\bbP = \tilde\bbP\circ(\Upsilon_i)^{-1}$, 
$(\tilde \phi_{k_i},\tilde \phi_{j_i}):= (\phi_{k_i}, \phi_{j_i}) \circ \Upsilon_i$ 
and \eqref{conv_skorohod} takes place, see \cref{Lem:Convergence}.

\noindent If we define $(\tilde \sigma_{k_i},\tilde \sigma_{j_i}):= (\sigma_{k_i}, \sigma_{j_i}) \circ \Upsilon_i$ 
and  $(\tilde \mu_{k_i},\tilde \mu_{j_i}):= (\mu_{k_i}, \mu_{j_i}) \circ \Upsilon_i$, 
the uniform bounds in \eqref{uniform_bounds_lambda} still holds  in the form
\begin{align*}
\norm{(\tilde \sigma_{k_i},\tilde \sigma_{j_i})}_{(L^p(\tilde\Omega;\! C^0([0,T];\! H)\cap L^2(0,T;\! V))\cap L^\infty(\Omega\times Q))^2} &\leq M, \\
\norm{(\tilde \phi_{k_i},\tilde \phi_{j_i})}_{(L^p(\tilde\Omega;\! C^0([0,T];\! H)\cap
L^\infty(0,T;\! V)\cap L^2(0,T;\! H^2_N(D))))^2} &\leq M , \\
\norm{(\tilde \mu_{k_i},\tilde \mu_{j_i})}_{(L^{p/2}(\tilde\Omega;\! L^2(0,T;\! V)))^2}+
\norm{\nabla (\tilde \mu_{k_i},\tilde \mu_{j_i})}_{(L^p(\tilde\Omega;\! L^2(0,T;\! H)))^2}
&\leq M ,\\
\norm{(\Psi'_\lambda(\tilde \phi_{k_i}),\Psi'_\lambda(\tilde \phi_{j_i}))}_{(L^{p/2}(\tilde\Omega;\! L^2(0,T;\! H)))^2} &\le M.
\end{align*}
This guarantees that,
up to passing to subsequences, 
recalling the strong convergence \eqref{conv_skorohod} and 
employing the strong-weak closure of maximal monotone operators
as well as the weak lower semicontinuity of the norms,
\begin{align*}
(\tilde \sigma_{k_i},\tilde \sigma_{j_i}) \rightharpoonup (\sigma^1, \sigma^2) 
\qquad &\text{ in } (L^p(\tilde\Omega;\! L^2(0,T;\! V)))^2, \\
(\tilde \sigma_{k_i},\tilde \sigma_{j_i}) \stackrel{*}{\rightharpoonup} (\sigma^1, \sigma^2) 
\qquad &\text{ in } (L^p(\tilde\Omega;\! L^1(0,T;\! H))^*\cap L^\infty(\tilde\Omega\times Q))^2,\\
(\tilde \phi_{k_i},\tilde \phi_{j_i}) \to (\phi^1, \phi^2) 
\qquad &\text{ in }  (L^\ell(\tilde\Omega;\! C^0([0,T];\! H)\cap L^2(0,T;\! V)))^2 
\quad\forall\ell\in[1,p), \\
(\tilde \phi_{k_i},\tilde \phi_{j_i}) \rightharpoonup (\phi^1, \phi^2) 
\qquad &\text{ in }  (L^p(\tilde\Omega;\! L^2(0,T;\! H^2_N(D))))^2, \\
(\tilde \mu_{k_i},\tilde \mu_{j_i}) \rightharpoonup (\mu^1, \mu^2) \qquad &\text{ in } (L^{p/2}(\tilde\Omega;\! L^2(0,T;\! V)))^2, \\
(\Psi'_\lambda(\tilde \phi_{k_i}),\Psi'_\lambda(\tilde \phi_{j_i})) \rightharpoonup (\Psi'(\phi^1), \Psi'(\phi^2)) \qquad &\text{ in } (L^{p/2}(\tilde \Omega;\! L^2(0,T;\! H)))^2,
\end{align*} 
where the limit objects belong  to the same spaces of the respective sequences.

\noindent Furthermore, for every $t \in [0,T]$ and $\tilde \bbP$-a.s. the following holds in $V'$, 
\begin{align*}
\partial_t (\tilde \phi_{k_i} - \tilde \phi_{j_i}) - \Delta(\tilde \mu_{k_i} - \tilde \mu_{j_i})  &= \mathcal P(\tilde \sigma_{k_i} - \tilde \sigma_{j_i}) h(\tilde \phi_{k_i}) +  (\mathcal P\tilde \sigma_{j_i} - a - \alpha u)\left( h(\tilde \phi_{k_i}) -  h(\tilde \phi_{j_i}) \right)\\
\tilde \mu_{k_i} - \tilde \mu_{j_i} &= - \Delta (\tilde \phi_{k_i} - \tilde \phi_{j_i}) + \Psi'(\tilde \phi_{k_i}) - \Psi'(\tilde \phi_{j_i}),
\end{align*}
and passing  to the limit as $i \to +\infty$ we get
\begin{align*}
\partial_t (\phi^1 - \phi^2) - \Delta(\mu^1 - \mu^2)  &= \mathcal P(\sigma^1 - \sigma^2) h(\phi^1) +  (\mathcal P \sigma^1 - a - \alpha u)\left( h(\phi^1) - h(\phi^2) \right)\\
\mu^1 - \mu^2 &= - \Delta (\phi^1 - \phi^2) + \Psi'( \phi^1) - \Psi'(\phi^2).
\end{align*}
From the uniqueness of the solution proved in Section~\ref{ssec:cont_dep} 
(see \eqref{uniquness_tau_N}, with $t \in [0,T]$) we deduce that $\phi^1(t) = \phi^2(t)$ 
for every $t \in [0,T]$, $\tilde \bbP$-a.s.~and this readily implies that 
$$ \nu \left(  \left\lbrace (g^1,g^2) \in (C^0([0,T];\! H) \cap L^2(0,T;\! V))^2 : g^1 = g^2 \right\rbrace \right) = \tilde \bbP (\phi^1= \phi^2) = 1,$$
and \eqref{crit_G-K} holds.
From Gy\"ongy-Krylov's criterion, see \cref{Lem:GyongyKrylov}, it holds that 
$$ \phil \to \phi \qquad  \text{ in } C^0([0,T];\! H) \cap L^2(0,T;\! V), \quad  \text{ in } \bbP\text{-measure on } \Omega.$$ 
Moreover, using the uniform bounds \eqref{uniform_bounds_lambda},
the lower semicontinuity of the norms and the strong-weak closure 
of maximal monotone graphs we also have that
\begin{align*}
\sigmal \stackrel{*}{\rightharpoonup} \sigma \qquad &\text{ in } L^p(\Omega;\! L^2(0,T;\! V))\cap L^\infty(\Omega\times Q), \\
\phil \to \phi \qquad &\text{ in }  L^\ell(\Omega;\! C^0([0,T];\! H)\cap L^2(0,T;\! V))
\quad\forall\ell\in[1,p), \\
\phil \rightharpoonup \phi \qquad &\text{ in }  L^p(\Omega;\!  L^2(0,T;\! H^2_N(D))),\\
\mul \rightharpoonup \mu \qquad &\text{ in } L^{p/2}(\Omega;\! L^2(0,T;\! V)),\\ 
\Psi'_\lambda(\phil) \rightharpoonup \Psi'(\phi) 
\qquad &\text{ in } L^{p/2}(\Omega;\! L^2(0,T;\! H)),
\end{align*}
where 
\begin{gather*}
\phi \in L^p(\Omega;\! C^0([0,T];\!H) \cap L^\infty(0,T;\! V)\cap L^2(0,T;\! H^2_N(D))), \\
\sigma \in L^p(\Omega;\! C^0([0,T];\! H)\cap L^2(0,T;\! V))\cap L^\infty(\Omega\times Q), \\
\mu \in L^{p/2}(\Omega;\! L^2(0,T;\!V)), \qquad
\nabla \mu \in L^p(\Omega;\! L^2(0,T;\!H)), \qquad \;\!(\mu)_D \in L^{p/2}(\Omega;\! L^\infty(0,T)), \\
\Psi'(\phi) \in L^{p/2}(\Omega;\! L^2(0,T;\!H)) .
\end{gather*}
Let us show a further convergence for $(\sigmal)_\lambda$.
To do it, we exploit the continuous dependence on data given in 
\eqref{eq:sigma_diff}. For every subsequences $\lambda_i, \lambda_j$, $i,j \in \bbN$
and every $\ell\in[1,p)$, it holds 
$$
   0 \leq 
   \norm{\sigma_{\lambda_i} - \sigma_{\lambda_j}}_{L^\ell\left(\Omega;\! C^0([0,T];\! H)
   \cap L^2(0,T;\! V)\right)} \lesssim 
   \norm{\phi_{\lambda_i} - \phi_{\lambda_j}}_{L^\ell(\Omega;\! L^2(0,T;\! H))} 
   \longrightarrow 0, 
$$
as $i \to \infty$.
This implies that $\sigma_{\lambda} \to \sigma$ in $L^\ell\left(\Omega;\! C^0([0,T];\! H)\cap 
L^2(0,T;\! V)\right)$, which allows to pass to the limit in the stochastic integrals, getting
by the Burkholder--Davis--Gundy inequality, see \cref{Lem:BurkholderDavisGundy}, that
$$
  \mathcal{H}(\sigma_{\lambda}) \cdot W_2 \to
   \mathcal{H}(\sigma) \cdot W_2\qquad\text{in } L^\ell(\Omega;\! C^0([0,T];\! H))
   \quad\forall\ell\in[1,p).
$$ 
Putting this information together and letting $\lambda\downarrow0$ in the approximated
problem, it is now straightforward to see that 
$(\phi,\mu,\sigma)$ is a solution to \eqref{phi1}--\eqref{eq_sigma_weak}.

